Knowledge Graph-based Question Answering with Electronic Health Records

Question Answering (QA) is a widely-used framework for developing and evaluating an intelligent machine. In this light, QA on Electronic Health Records (EHR), namely EHR QA, can work as a crucial milestone towards developing an intelligent agent in healthcare. EHR data are typically stored in a relational database, which can also be converted to a directed acyclic graph, allowing two approaches for EHR QA: Table-based QA and Knowledge Graph-based QA. We hypothesize that the graph-based approach is more suitable for EHR QA as graphs can represent relations between entities and values more naturally compared to tables, which essentially require JOIN operations. In this paper, we propose a graph-based EHR QA where natural language queries are converted to SPARQL instead of SQL. To validate our hypothesis, we create four EHR QA datasets (graph-based VS table-based, and simplified database schema VS original database schema), based on a table-based dataset MIMICSQL. We test both a simple Seq2Seq model and a state-of-the-art EHR QA model on all datasets where the graph-based datasets facilitated up to 34% higher accuracy than the table-based dataset without any modification to the model architectures. Finally, all datasets are open-sourced to encourage further EHR QA research in both directions.

==> tables/correct_per_join.tex <==

 
\begin{wraptable}{r}{0.73\textwidth}
\caption{The number of correctly generated queries for test questions binned by the number of \textit{JOIN}s in the SQLs of \sqlset. The SPARQLs are classified without \textit{JOIN}s because both queries are derived from the same question}
\label{tab:correct_per_join}
% \resizebox{\columnwidth}{!}{%
\centering
\small

\begin{tabular}{llcccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} &
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} &
\multicolumn{1}{c}{\textbf{Dataset}} &
\multicolumn{6}{c}{\textbf{ \# of \textit{INNER JOIN}}s} \\
& \multicolumn{1}{c}{Simplified Schema} & 0 & 1& 2 & 3 & 4 & 5 \\
\midrule

\multirow{2}{*}{Seq2Seq} 
 & \mimicsql & 123 & 33 & 0 & - & - & - \\ 
 & \mimicsparql & \textbf{209} & \textbf{89} & 0 & - & - & - \\
 \cmidrule(lr){2-8}
 \multirow{2}{*}{TREQS} 
 & \mimicsql & \textbf{383} & \textbf{271} & 4 & - & - & - \\ 
 & \mimicsparql & 376 & 265 & \textbf{5} & - & - & - \\
 \midrule
 \multicolumn{2}{c}{\textbf{\# of questions per \textit{INNER JOIN}s}}  &  528 & 450 & 22 & - & - & - \\
\bottomrule
\end{tabular}  

\vspace{3mm}

\begin{tabular}{llcccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} &
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} &
\multicolumn{1}{c}{\textbf{Dataset}} &
\multicolumn{6}{c}{\textbf{ \# of \textit{INNER JOIN}}s} \\
& \multicolumn{1}{c}{Original Schema} & 0 & 1& 2 & 3 & 4 & 5 \\
\midrule

\multirow{2}{*}{Seq2Seq} 
 & \sqlset & \textbf{37} & 134 & 21 & 17 & 0 & 0 \\ 
 & \sparqlset & 29 & \textbf{180} & \textbf{43} & \textbf{31} & \textbf{2} & 0 \\ 
 \cmidrule(lr){2-8}
\multirow{2}{*}{TREQS} 
 & \sqlset & 79 & 276 & 145 & 93 & \textbf{2} & 0 \\ 
 & \sparqlset & 79 & \textbf{289} & \textbf{163} & \textbf{111} & 1 & 0 \\ 
 \midrule
 \multicolumn{2}{c}{\textbf{\# of questions per \textit{INNER JOIN}s}}  &  130 & 398 & 214 & 236 & 2 & 5 \\
 
\bottomrule
\end{tabular}

\end{wraptable}
